Analyzing a Tandem Fluid Queueing Model with Stochastic Capacity and Spillback

The tandem fluid queueing model is a useful tool for performance analysis and control design for a variety of transportation systems. In this article, we study the joint impact of stochastic capacity and spillback on the long-time properties of this model. Our analysis focuses on the system of two fluid queueing links in series. The upstream link has a constant capacity (saturation rate) and an infinite buffer size. The downstream link has a stochastic capacity and a finite buffer size. Queue spillback occurs when the the downstream link is full. We derive a necessary condition and a sufficient condition for the total queue length to be bounded on average. The necessary (resp. sufficient) condition leads to an upper (resp. lower) bound for the throughput of the two-link system. Using our results, we analyze the sensitivity of throughput of the two-link system with respect to the frequency and intensity of capacity disruptions, and to the buffer size. In addition, we discuss how our analysis can be extended to feedback-controlled systems and to networks consisting of merges and splits.

==> Texts/10_Intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 1 page
\section{Introduction}

Capacity fluctuations is common in transportation systems.
Typical examples include incidents on freeways \cite{skabardonis97,schrank12} and weather-related capacity drops at airports \cite{peterson95,ny11}.
In many cases, capacity fluctuations are frequent and hard to predict deterministically \cite{skabardonis97,peterson95,jin17}.
Consequently, throughput analysis under stochastic capacity is relevant for transportation system operators.

Some authors pointed out that throughput of a transportation system is also affected by congestion propagation within the system, i.e. queue spillback \cite{daganzo98,papageorgiou03,shen14}. Queue spillback may lead to traffic queues in the upstream links of a bottleneck, which may give rise to additional bottlenecks in this upstream links. 
Consequently, spillback may also lead to capacity loss.
%Consequently, spillback may add to the throughput loss due to capacity fluctuation. However, limited work has been done to estimate the throughput loss due to both capacity fluctuation and spillback.

The impact of stochastic capacity and that of spillback have been studied by two relatively independent lines of work \cite{kulkarni97,shen14}.
In this article, we use a simple fluid queueing model to study the joint impact of these two factors, which provides new insights for operations of transportation systems.

This class of models have been extensively used for analysis of transportation systems \cite{kulkarni97,daganzo98,newell13}.
Specifically, we consider two fluid queueing links in series, where a constant inflow is sent to the upstream link.
The downstream link has a stochastically varying capacity and a finite buffer size. Queue spillback happens when the downstream link is full.
Following \cite{dai95}, we consider the two-link system to be stable if the total queue length is bounded on average.
We view the supremum of the set of stable inflows as the throughput.
Our objective is to derive stability conditions for the two-link system, which leads to bounds on the throughput.
Although we are motivated by transportation applications, our model and method are also relevant for communication networks and manufacturing systems \cite{kulkarni97,yu04}.

Fluid queueing systems with stochastic capacities have been studied previously; see \cite{anick82,chen92,kella92,kulkarni97,whitt02} for notable contributions.
This line of work focuses on the analysis of the stationary distribution of queue length in a single link. 
An important conclusion from this line of work is that a single fluid queueing link is stable if and only if the inflow is less than the time-average capacity \cite{kulkarni97}.
However, due to queue spillback, this conclusion does not directly extend to multiple links in series.
An important insight from our analysis is that a system of multiple fluid queueing links in series is not necessarily stable even if the inflow is strictly less than the time-average capacity of every link.

The main results of this article (Propositions~\ref{Prp_Stable1} and \ref{Prp_Stable2}) provide stability conditions for the two-link system.
The stability conditions build on known results on stability analysis of continuous-time Markov processes \cite{davis84,meyn93} and steady-state behavior of stochastic fluid queueing models \cite{anick82,kulkarni97,jin16}.

First, a necessary condition is derived based on known results on the steady-state behavior of single fluid queueing links with finite buffer sizes \cite{anick82,kulkarni97}.


Our work builds on known results on stability analysis of continuous-time Markov processes \cite{meyn93,meyn93ii,cloez15} and properties of PDMPs \cite{davis84,benaim15}.
A necessary condition for a Markov process to be stable is that the process is {non-evanescent}, i.e. that the state is finite almost surely.
A sufficient condition is that the process admits a {Lyapunov function} satisfying the Foster-Lyapunov drift condition \cite{meyn93} and has a unique invariant probability measure.
We build on the above results and derive stability conditions that can be directly applied to feedback controlled PDQs.
We show that, in general, there is a gap between the necessary condition and the sufficient condition; however, under particular assumptions, these conditions are equivalent.

In Section~\ref{Sec_PDQ}, we derive a necessary condition (Theorem~\ref{Thm_PDQ1}) and a sufficient condition (Theorem~\ref{Thm_PDQ2}) for the stability of feedback-controlled PDQs. The necessary condition is that the time-average inflow does not exceed the time-average saturation rate. The sufficient condition requires the infima of the control policy in various modes to verify a bilinear matrix inequality (BMI), which essentially imposes a bound on the controlled inflow.
The BMI results from the application of the Foster-Lyapunov drift condition to our setting with a suitably chosen Lyapunov function.
The sufficient condition also restricts the form of the control policy to ensure the uniqueness of the invariant probability measure.
Importantly, our sufficient condition also leads to an estimate of an exponential rate of convergence towards the invariant probability measure.
We use these results to study the stability of several practically relevant control policies, including mode-responsive and linear feedback control policies.

In Section~\ref{Sec_BPDQ}, we analyze PDQs with two modes, or \emph{bimodal} PDQs (BPDQs).
These simpler systems are of practical interest, since they can model traffic links that stochastically switch between a nominal mode and a disrupted mode (with reduced or zero capacity).
In addition, our analysis of BPDQs provides a clear intuition and some useful insights.
The main result of this section (Theorem~\ref{Thm_BPDQ}) is that a controlled BPDQ is stable if and only if a weighted average of the infima of the control policy in various modes is less than the average saturation rate.
In addition, for stable BPDQs, we are able to derive bounds on the steady-state queue length and the exponential rate of convergence to the invariant probability measure, in terms of the model parameters and characteristics of the control policy.

In Section~\ref{Sec_Net}, we illustrate some applications of our results to traffic routing under stochastic capacity fluctuation.
We consider the stability of typical traffic routing policies over a network of two links in parallel.
We apply our results to analyze the stability of static and mode-responsive routing policies. Under particular assumptions, we also compute optimal routing policies that minimize the expected travel time. 
Finally, we study the stability and performance of the well-known logit routing model \cite{como13i,benakiva84}, which, for our purposes, can be viewed as a queue-responsive routing policy.
% queue-responsive routing, we consider the commonly used logit routing model \cite{como13i,benakiva84}, and show its stability in the setting of stochastically switching capacities.

==> Texts/10_Intro2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 1 page
\section{Introduction}

Capacity fluctuations is common in transportation systems.
Typical examples include incidents on freeways \cite{skabardonis97,schrank12} and weather-related capacity drops at airports \cite{peterson95,ny11}.
In many cases, capacity fluctuations are frequent and hard to predict deterministically \cite{skabardonis97,peterson95,jin17}.
Consequently, throughput analysis under stochastic capacity is relevant for transportation system operators.

Some authors pointed out that throughput of a transportation system is also affected by congestion propagation within the system, i.e. queue spillback \cite{papageorgiou03}. Queue spillback may lead to traffic queues in the upstream links of a bottleneck, which may give rise to additional bottlenecks in this upstream links. Consequently, spillback may add to the throughput loss due to capacity fluctuation. However, limited work has been done to estimate the throughput loss due to both capacity fluctuation and spillback.

In this article, we use a simple fluid queueing model to study the joint impact of capacity fluctuation and queue spillback.
This class of models have been extensively used for analysis of transportation systems \cite{kulkarni97,daganzo98,newell13}.
Specifically, we consider two fluid queueing links in series, where a constant inflow is sent to the upstream link.
The downstream link has a stochastically varying capacity and a finite buffer size. Queue spillback happens when the downstream link is full.
Following \cite{dai95}, we consider the two-link system to be stable if the total queue length is bounded on average.
We view the supremum of the set of stable inflows as the throughput.
Our objective is to derive stability conditions for the two-link system, which leads to bounds on the throughput.
Although we are motivated by transportation applications, our model and method are also relevant for communication networks and manufacturing systems \cite{kulkarni97,yu04}.

Fluid queueing systems with stochastic capacities have been studied previously; see \cite{anick82,chen92,kella92,kulkarni97,whitt02} for notable contributions.
This line of work focuses on the analysis of the stationary distribution of queue length in a single link. 
An important conclusion from this line of work is that a single fluid queueing link is stable if and only if the inflow is less than the time-average capacity \cite{kulkarni97}.
However, due to queue spillback, this conclusion does not directly extend to multiple links with interaction.
An important insight from our analysis is that a system of multiple fluid queueing links in series is not necessarily stable even if the inflow is strictly less than the time-average capacity of every link.

The main results of this article (Propositions~\ref{Prp_Stable1} and \ref{Prp_Stable2}) provide stability conditions for the two-link system.
The stability conditions build on known results on stability analysis of continuous-time Markov processes \cite{davis84,meyn93} and steady-state behavior of stochastic fluid queueing models \cite{anick82,kulkarni97,jin16}.

First, a necessary condition is derived based on known results on the steady-state behavior of single fluid queueing links with finite buffer sizes \cite{anick82,kulkarni97}.


Our work builds on known results on stability analysis of continuous-time Markov processes \cite{meyn93,meyn93ii,cloez15} and properties of PDMPs \cite{davis84,benaim15}.
A necessary condition for a Markov process to be stable is that the process is {non-evanescent}, i.e. that the state is finite almost surely.
A sufficient condition is that the process admits a {Lyapunov function} satisfying the Foster-Lyapunov drift condition \cite{meyn93} and has a unique invariant probability measure.
We build on the above results and derive stability conditions that can be directly applied to feedback controlled PDQs.
We show that, in general, there is a gap between the necessary condition and the sufficient condition; however, under particular assumptions, these conditions are equivalent.

In Section~\ref{Sec_PDQ}, we derive a necessary condition (Theorem~\ref{Thm_PDQ1}) and a sufficient condition (Theorem~\ref{Thm_PDQ2}) for the stability of feedback-controlled PDQs. The necessary condition is that the time-average inflow does not exceed the time-average saturation rate. The sufficient condition requires the infima of the control policy in various modes to verify a bilinear matrix inequality (BMI), which essentially imposes a bound on the controlled inflow.
The BMI results from the application of the Foster-Lyapunov drift condition to our setting with a suitably chosen Lyapunov function.
The sufficient condition also restricts the form of the control policy to ensure the uniqueness of the invariant probability measure.
Importantly, our sufficient condition also leads to an estimate of an exponential rate of convergence towards the invariant probability measure.
We use these results to study the stability of several practically relevant control policies, including mode-responsive and linear feedback control policies.

In Section~\ref{Sec_BPDQ}, we analyze PDQs with two modes, or \emph{bimodal} PDQs (BPDQs).
These simpler systems are of practical interest, since they can model traffic links that stochastically switch between a nominal mode and a disrupted mode (with reduced or zero capacity).
In addition, our analysis of BPDQs provides a clear intuition and some useful insights.
The main result of this section (Theorem~\ref{Thm_BPDQ}) is that a controlled BPDQ is stable if and only if a weighted average of the infima of the control policy in various modes is less than the average saturation rate.
In addition, for stable BPDQs, we are able to derive bounds on the steady-state queue length and the exponential rate of convergence to the invariant probability measure, in terms of the model parameters and characteristics of the control policy.

In Section~\ref{Sec_Net}, we illustrate some applications of our results to traffic routing under stochastic capacity fluctuation.
We consider the stability of typical traffic routing policies over a network of two links in parallel.
We apply our results to analyze the stability of static and mode-responsive routing policies. Under particular assumptions, we also compute optimal routing policies that minimize the expected travel time. 
Finally, we study the stability and performance of the well-known logit routing model \cite{como13i,benakiva84}, which, for our purposes, can be viewed as a queue-responsive routing policy.
% queue-responsive routing, we consider the commonly used logit routing model \cite{como13i,benakiva84}, and show its stability in the setting of stochastically switching capacities.

==> Texts/48_Resilience.tex <==
\section{Resilience interpretation}
\label{Sec_Resilience}

Now we argue that our results are also relevant for resilience analysis of transportation systems.

In reality, accurate estimate of buffer size $\theta$ is not always an easy task.
Inaccurate data reported by traffic sensors leads to inaccurate estimate of $\theta$.
Corrupted or manipulated data lead to inaccurate estimate of the buffer size.

The resilience of the two-link system can be measured by the maximum misjudgment of the buffer size that does not affect stability.
Our model can be applied to estimate this resilience metric.

Suppose that, based on traffic sensor data, a traffic manager determines the buffer size to be $\hat\theta$, and, accordingly, sets the inflow to be $\hat r$.
Note that, for each inflow $r\in\R$, we can determine a threshold for buffer size with stability guarantee. That is, for each given $r$, we can obtain from Proposition~\ref{Prp_Stable2} a quantity $\theta_\min(r)$ such that, for each $\theta\ge\theta_\min(r)$, the two-link system is guaranteed to be stable.
Then, the following quantity measures the resilience:
\begin{align*}
\alpha(\hat r)=\frac{\hat\theta-\theta_\min(\hat r)}{\hat\theta},\quad
\hat r\le\overline r.
\end{align*}
In other words, $\alpha=1$ if any estimate error for the buffer size can be tolerated; $\alpha=0$ if no estimate error can be tolerated.

\begin{figure}[hbt]
\centering
\includegraphics[width=0.45\textwidth]{./Images/Fig_thetamin}
\caption{.}
\label{Fig_thetamin}
\end{figure}

We numerically compute $\theta_\min(r)$ and thus $\alpha(\hat r)$ for various values of $\hat r$, which is shown in Figure~\ref{Fig_thetamin}. For each $\hat r\in[0, 0.625]$, the two-link system is necessarily stable, regardless of the buffer size. For each $\hat r\in(0.625,0.684)$, there exists a positive amount of misjudgment that can be tolerated. For $\hat r\ge0.684$, our results do not provide guarantee for stability.

==> Texts/49_Net__Li_Jin_s_conflicted_copy_2017-03-18_.tex <==
\section{Extension to merges and splits}
\label{Sec_Net}

Now we discuss how our approach can be extended from the two-link system to merges and splits.
This discussion is helpful to understand the behavior of more general fluid queueing networks with finite buffer sizes.

\subsection{Merges}
Consider a merge, i.e. three fluid queueing links connected as in Figure~\ref{Fig_Merge}. Links 1 and 2 have constant capacities and infinite buffer size. Link 3 has a capacity switching between $u_1$ and $u_2$, and a buffer size of $\theta$.
The state space is $\Q_m=[0,\infty)^2\times[0,\theta]$.

We assume that flow from link 1 is prioritized over link 2.
Consider the following Lyapunov function:
\begin{align*}
V_m(i,q)=q_1^2+a_{1,i}q_1q_3+b_{1,i}q_1
+q_2^2+a_{2,i}q_2q_3+b_{2,i}q_2,
\end{align*}
where $a_{1,i}$, $a_{2,i}$, $b_{1,i}$, and $b_{2,i}$ are positive constants.
Applying the infinitesimal generator of the merge, we have
\begin{align*}
&\Ell V_m(1,q)\\
&=(2\dot q_1+a_{1,1}\dot q_3+\lambda(a_{1,2}-a_{1,1})q_3+\lambda(b_{1,2}-b_{1,1}))q_1\\
&\quad+(2\dot q_2+a_{2,1}\dot q_3+\lambda(a_{2,2}-a_{2,1})q_3+\lambda(b_{2,2}-b_{2,1}))q_2\\
&\quad+(a_{1,1}\dot q_1+a_{2,1}\dot q_2)+b_{1,1}\dot q_1+b_{2,1}\dot q_2.\\
&\Ell V_m(1,q)\\
&=(2\dot q_1+a_{1,1}\dot q_3+\lambda(a_{1,2}-a_{1,1})q_3+\lambda(b_{1,2}-b_{1,1}))q_1\\
&\quad+(2\dot q_2+a_{2,1}\dot q_3+\lambda(a_{2,2}-a_{2,1})q_3+\lambda(b_{2,2}-b_{2,1}))q_2\\
&\quad+(a_{1,1}\dot q_1+a_{2,1}\dot q_2)+b_{1,1}\dot q_1+b_{2,1}\dot q_2.
\end{align*}
Then, 

The behavior of a merge is similar to that of the two-link system. However, an important distinct property of a merge is that stability not only depends on the sum of the inflows, but also how the inflows are distributed over the upstream links.

\subsection{Splits}
Consider a split, i.e. three fluid queueing links connected as in Figure~\ref{Fig_Merge}. For ease of presentation, we assume that links 1 and 2 have constant capacities and infinite buffer size, while link 3 has a capacity switching between $u_1$ and $u_2$, and a buffer size of $\theta$.

We assume that flow from link 1 is prioritized over link 2.

The most important property of a split is that congestion in one downstream link may undermines the efficiency in the other downstream link.

==> Texts/60_Appx.tex <==
\begin{appendices}
\renewcommand{\theequation}{\Alph{section}.\arabic{equation}}
{\footnotesize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{{\footnotesize} Network stability conditions}
\label{Sub_Net}

\begin{proof}[Proof of Thm \ref{Thm_Capacity}]
Consider an arbitrary link $\e\in\edge$. If the network is stable, then link $\e$ is stable in the sense that the law of $q_\e(t)$ converges to a unique invariant marginal distribution. Therefore, $\Pr\{\lim_{t\to\infty}q_\e(t)=\infty\}=0$. By Prop.~\ref{Prp_Capacity}, we know $\overline\phi_\e\le\ubar_\e$. Since the argument above applies to any link $\e\in\edge$, we deduce that $\overline\bfphi\le\overline\bfu$.
\end{proof}

\begin{proof}[Proof of Thm. \ref{Thm_Net}]
To show the drift condition, consider the Lyapunov function defined as
\begin{align*}
V(i,\bfq)=k_i e^{\bfb^T \bfq},\; i\in\I.
\end{align*}
Let $\bfV(\bfq)=[V(1,\bfq),\ldots,V(z,\bfq)]^T=\Big(e^{\bfb^T \bfq}\Big)\bfk$.
By \eqref{Eq_Lgiq}, we have
\begin{align*}
\Ell\bfV(\bfq)=\Bigg(\diag\bigg(\Big(\bfPhi^T(\bfq)-\bfR^T(\bfq,\bfphi)\Big)\bfb\bigg)+\bfLmd\Bigg) \Big(e^{\bfb^T \bfq}\Big)\bfk,
\end{align*}
where $\Ell\bfV(\bfq)=[\Ell V(1,\bfq),\ldots,\Ell V(z,\bfq)]^T$.
Then \eqref{Eq_phiijkb} ensures that there exists $C=\min_{i\in\I}1/k_i$ such that
\begin{align*}
\Ell\bfV(\bfq)\le -C\bfV(\bfq),\;\forall\bfq\in\real_+^m\backslash\{\bf0\}.
\end{align*}
To cover the case where $\bfq=\bf0$, let
\begin{align*}
K=\max_{i\in\I}\|\Ell\bfV({\bf0})+C\bfV(\mathbf0)\|_1,
\end{align*}
where $\|\cdot\|_1$ is the 1-norm of vectors. Then, one can show that
\begin{align*}
\Ell\bfV({\bf0})\le K\bfe-C\bfV(\mathbf0).
\end{align*}
Thus, we conclude that
\begin{align*}
\Ell\bfV(\bfq)\le K\bfe-\bfV(\bfq),\;\forall\bfq\in\real_+^m.
\end{align*}
Hence, with $\varphi(x)=C\log(x+1)$, we have the drift condition
\begin{align*}
\Ell V(i,\bfq)\le K-\varphi\Big(V(i,\bfq)\Big),\;\forall (i,\bfq)\in\I\times\real_+^m.
\end{align*}

For the minorization condition, following the procedure presented in the proof of Prop.~\ref{Prp_Individual}, one can show that, for any initial condition $(i_0,\bfq_0)\in\I\times\real_+^m$, there is a strictly positive probability that, after a sufficiently long but finite time, the system resides exactly at $(i^*,\mathbf 0)$. To see the finiteness of such a time, note that, for $\bfq\neq\bf0$, $d\Big(\bfq^T\bfe\Big)/dt=\Big(\bfphi(i^*,\bfq)-\bfr(\bfphi,i^*,\bfq)\Big)^T\bfe\le-\epsilon<0$. Hence, in mode $i^*$ the queues will vanish within finite time.
This implies the minorization condition.

With the above two conditions satisfied, we conclude that the PDQ network with routing policy $\bfphi$ is stable.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{{\footnotesize} Stability conditions under particular assumptions}
\label{Sub_Particular}

\subsubsection{{\footnotesize} Non-interacting links}

In this case, stability of the network is almost equivalent to the stability of individual queues.
For a static routing policy $\bfphi_\bfGmm\in\real_+^m$, we have
$
\bfd=\bfphi_\bfGmm.
$
The static routing policy $\bfphi_\bfGmm$ is admissible if
\begin{align*}
\bfe_1+\bfA\bfphi_\bfGmm-\bfB\bfphi_\bfGmm=\mathbf 0.
\end{align*}


For a mode-dependent routing policy $\bfphi_\bfEta:\I\to\real_+^m$, we can represent $\bfphi_\bfEta$ with the $m\times z$ constant matrix
\begin{align}
\bfPhi_\bfEta&=\Big[
\bfphi_\bfEta(1) | \bfphi_\bfEta(2) |\ldots | \bfphi_\bfEta(z)
\Big]
\label{Eq_bfPhi2}
\end{align}
The outflow vector is given by
$
\bfd=\bfPhi_\bfEta\sfp^T.
$
Let $\bfD=\bfPhi_\bfEta\sfp^T\bfe^T$ and one can show that the mode-dependent policy is admissible if
\begin{align*}
\bfe_1\bfe^T+\bfA\bfD-\bfB\bfPhi_\bfEta=\mathbf 0.
\end{align*}

The following result particularizes Thm.~\ref{Thm_Net} for PDQ networks with non-interacting links under static/mode-dependent routing policies.

\begin{cor}
\label{Cor_d}
A PDQ network $\la\I,\Q,\F,\Init,P\ra$ with constant $\bfd$ and with an admissible, mode-dependent policy $\bfphi_\bfEta:\I\to\real_+^m$ is stable if there exist constant vectors $\bfb>0$ and $\bfk>0$ such that
\begin{align}
\Bigg(\diag\bigg(\Big(\bfPhi_\bfEta^T-\bfR^T(\bfq,\bfphi_\bfEta)\Big)\bfb\bigg)+\bfLmd\Bigg)\bfk\le-\bfe,\;
\forall \bfq\in\real_+^m,
\label{Eq_etakb}
\end{align}
where $\bfPhi$ and $\bfR$ are as defined in \eqref{Eq_bfPhi2} and \eqref{Eq_bfR}, respectively.
Furthermore, if the routing policy is static and is represented by a flow vector $\bfphi_\bfGmm\in\real_+^m$, then the network is stable if there exist constant vectors $\bfb>0$ and $\bfk\ge0$ such that
    \begin{align*}
    \Bigg(\diag\bigg(\Big(\bfe\bfphi_\bfGmm^T-\bfR^T(\bfq,\bfphi_\bfGmm)\Big)\bfb\bigg)+\bfLmd\Bigg)\bfk\le-\bfe,\;
    \forall \bfq\in\real_+^m.
%            \label{Eq_gammakb}
    \end{align*}
\end{cor}

The number of independent inequalities that \eqref{Eq_etakb} leads to depends on how complex the PDQ network is. For every $\bfq\in\real_+^m$, \eqref{Eq_etakb} represents $z$ inequalities. Note that $\bfR(\bfq)$ can take no more than $2^m$ values. 
%Thus, given $\bfGmm$, $\bfR(\bfq,\bfphi)$ cannot take more than $2^m$ values. 
Therefore, \eqref{Eq_etakb} leads to no more than $(2^m)z$ bilinear inequalities about $(z+m)$ independent variables.



%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{{\footnotesize} Interacting links}

If $\bfd(i,\bfq,\bfphi)=\bfr(i,\bfq,\bfphi)$, for a static routing policy $\bfphi_\bfGmm\in\real_+^m$ associated with the constant matrix $\bfGmm\in\real_+^{m\times n}$, we have
\begin{align*}
\bfPhi_\bfGmm(\bfq)=\bfGmm\Big(\bfA\bfR(\bfq,\bfphi_\bfGmm)+\bfe_1\bfe^T\Big),
\end{align*}
One way to find $\bfR$ is to solve the set of inequalities
\begin{align*}
&\bfe_1\bfe^T+\bfA\bfR(\bfq,\bfphi_\bfGmm)-\bfB\bfGmm\Big(\bfA\bfR(\bfq,\bfphi_\bfGmm)+\bfe_1\bfe^T\Big)=\mathbf0,\\
&\bfR(\bfq,\bfphi_\bfGmm)\le\bfU,\;
\bfR(\bfq,\bfphi_\bfGmm)\ge\bfS(\bfq)\bfU,
\end{align*}
where $\bfS(\bfq)=\diag\Big(\sgn(q_1),\ldots,\sgn(q_m)\Big)$.
%Thus, we have
%\begin{align*}
%\Ell\bfg(\bfq)=\bigg(\bfR^T(\bfGmm,\bfq)\Big(\bfA^T\bfGmm^T-\bfI\Big)+\bfE_1^T\bfGmm^T\bigg)\bfJ_\bfq(\bfg)+\bfLmd\bfg(\bfq).
%\end{align*}

For a mode-dependent routing policy $\bfphi_\bfEta:\I\times\real_+^m\to\real_+^m$ associated with a matrix-valued function $\bfEta:\I\to\real_+^{m\times n}$, we have
\begin{align*}
\bfphi_\bfEta(i,\bfq)=\bfEta(i)\Big(\bfA\bfr(i,\bfq,\bfphi_\bfEta)+\bfe_1\Big),\; (i,\bfq)\in\I\times\real_+^m.
\end{align*}

The following result particularizes Thm.~\ref{Thm_Net} for PDQ networks with interacting links under static/mode-dependent routing policies.

\begin{cor}
\label{Cor_dr}
A PDQ network$\la\I,\Q,\F,\Init,P\ra$ with $\bfd=\bfr$ and with an admissible, mode-dependent policy $\bfphi_\bfEta$ is stable if there exist constant vectors $\bfb>\mathbf0$ and $\bfk>\mathbf0$ such that, for all $\bfq\in\real_+^m\backslash\{\bf0\}$,
            \begin{align*}
            \Bigg(\diag\bigg(\Big(\bfPhi_\bfEta^T(\bfq)-\bfR^T(\bfq,\bfphi_\bfEta)\Big)\bfb\bigg)+\bfLmd\Bigg)\bfk\le-\bfe.
            \end{align*}
Furthermore, if the routing policy is static and is represented by a constant matrix $\bfGmm\in\real_+^{m\times n}$, then the network is stable if there exist constant vectors $\bfb>0$ and $\bfk>0$ such that, for all $\bfq\in\real_+^m\backslash\{\bf0\}$,
            \begin{align*}
            \Bigg(\diag\bigg(\Big(\bfR^T(\bfq,\bfphi_\bfGmm)(\bfA^T\bfGmm^T-\bfI)+\bfe\bfe_1^T\bfGmm^T\Big)\bfb\bigg)+\bfLmd\Bigg)\bfk\\\le-\bfe
%            \label{Eq_gammakb}
            \end{align*}
            where $\bfR$ is as defined in \eqref{Eq_bfR} and $\bfI$ is the identity matrix.
\end{cor}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{{\footnotesize} Stability condition for BPDQs}
\label{Sub_Convergence2}
\begin{proof}[Proof of Prop.~\ref{Prp_Convergence2}]
By Prop.~\ref{Prp_Capacity}, if a BPDQ is stable, then $f\le\ubar$. To rule out the case of $f=\ubar$, note that, if $f=\ubar$, then the limiting fraction of time of $q(t)=0$ is exactly zero; otherwise \eqref{Eq_lim3} would imply that $q(t)$ grows unboundedly. Thus, if the BPDQ admitted an invariant probability measure $p_f$ supported over some subset of $\I\times\real_+^m$, then we would have $p_f(i,\{0\})=0$ for all $i\in\{1,2\}$. However, for any $(i_0,q_0)\in\Init$, since $f<u^1$ (note that $f=\ubar<u^1$), there exists a finite $T>0$ such that $P_T\Big((i_0,q_0),(1,\{0\})\Big)>0$. Thus, if $p_f(i,\{0\})=0$, then $p_f$ could not be invariant with respect to $P_T$, which is a contradiction.

To show the converse, we argue that the system is stable if $f<\ubar$. If $f\le u^2$, the queue never grows, and thus the proof is trivial. If $u^2<f<\ubar$, we have
\begin{align*}
F-U=[f-u^1,f-u^2]^T,\;
\bfLmd=\left[\begin{array}{cc}
-\lambda&\lambda\\
\mu&-\mu
\end{array}\right].
\end{align*}
Thus, we can write
\begin{align*}
(F-U)b+\bfLmd=\left[\begin{array}{cc}
b(f-u^1)-\lambda&\lambda\\
\mu&b(f-u^2)-\mu
\end{array}\right],
\end{align*}
and
\begin{align}
\mathrm{det}[(F-U)b+\bfLmd]=&b^2(f-u^1)(f-u^2)\nonumber\\
&-\lambda b(f-u^2)-\mu b(f-u^1).
\label{Eq_det}
\end{align}
We can compute the steady state probabilities of $i$ by \eqref{Eq_pLmd}, which yields
\begin{align}
\sfp_1=\frac{\mu}{\lambda+\mu},\;
\sfp_2=\frac{\lambda}{\lambda+\mu},
\label{Eq_p1p2}
\end{align}
Then, by Prop.~\ref{Prp_Capacity}, we obtain \eqref{Eq_ubar12}.
%\begin{align*}
%\ubar=\frac{\mu u^1+\lambda u^2}{\lambda+\mu}.
%\end{align*}
Combining \eqref{Eq_ubar12} and \eqref{Eq_det} , we have
\begin{align*}
\det[(F-U)b+\bfLmd]=b^2(f-u^1)(f-u^2)+(\lambda+\mu)b(\ubar-f).
\end{align*}
Since $u^2<f<\ubar$, we have $f-u^1<0$, $f-u^2>0$, and $f-\ubar>0$. Hence, if
\begin{align}
0<b<\frac{(\lambda+\mu)(\ubar-f)}{-(f-u^1)(f-u^2)},
\label{Eq_b1}
\end{align}
then $\det[(F-U)b+\bfLmd]>0$ and $[(F-U)b+\bfLmd]$ is thus invertible.
By Cramer's rule, the solution to $[bF+\bfLmd]\bfk=-\bfe$ is given by
\begin{align*}
k_1=\frac{-(f-u^2)b+\lambda+\mu}{\det[(F-U)b+\bfLmd]},\;
k_2=\frac{-(f-u^1)b+\lambda+\mu}{\det[(F-U)b+\bfLmd]}.
\end{align*}
Since $f<u^1$, $k_2$ is positive. To ensure that $k_1>0$, we need
\begin{align}
0<b<\frac{\lambda+\mu}{f-u^2}.
\label{Eq_b2}
\end{align}
Since $f<\ubar<u^1$, \eqref{Eq_b2} naturally follows from \eqref{Eq_b1}. In conclusion, if $u^2<f<\ubar$, then there exists $b$ satisfying \eqref{Eq_b1} and thus \eqref{Eq_fkb}. By Corr.~\ref{Cor_Convergence}, the BPDQ system is stable, which completes the proof.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{{\footnotesize} Derivation of invariant probability measure}
\label{Sub_Fp}
Consider a PDQ (with possibly more than two modes), and any smooth function $g:\I\times\real_+\to\real$.
Recalling definitions of $\Phi$, $R$, $\bfg$, $\bfLmd$, and $\bfp_\phi$ from Sec.~\ref{Sub_Model} and noting that $q$ and $\phi$ are scalar-valued, we can expand \eqref{Eq_sumLg} as
\begin{align*}
&\sum_{i\in\I}\int_{dq\in\Q}\Ell g(i,q)p_\phi(i,dq)
=\int_{dq\in\Q}\bigg(\diag\Big(\Phi(q)\\
&\hspace{2cm}-R(\phi,q)\Big)\frac{d\bfg(q)}{dq}+\bfLmd\bfg(q)\bigg)^T\bfp_\phi(dq)
=0.
\end{align*}
An intuitive observation is that $p_\phi(i,q)$ may consist of a probability mass at $q=0$ and a scaled probability density over $[0,\infty)$, since there may be some fraction of time that the system sees no queue.
Therefore, we write $p_\phi(i,dq)=\sfz_i\delta_0dq+\sff_{i}(q)dq$, where $\sfz_i$ is the fraction of time that the system sees no queues in mode $i$, $\sff_i(q)$ is a bounded, non-negative function, and $\delta_0$ is the Dirac delta function centered at 0.
Let $\bfz=[\sfz_1,\ldots,\sfz_z]^T$ and $\mathbb{f}(q)=[\sff_1(q),\ldots,\sff_z(q)]^T$, and we have
\begin{align}
&\sum_{i\in\I}\int_{dq\in\Q}\Ell g(i,q)p_\phi(i,dq)\nonumber\\
&=\bigg(\diag\Big(\Phi(0)-R(\phi,0)\Big)\frac{d\bfg(q)}{dq}\bigg|_{q=0}+\bfLmd\bfg(0)\bigg)^T\bfz\nonumber\\
&+\int_{q\in\Q}\bigg(\diag\Big(\Phi(q)-R(\phi,q)\Big)\frac{d\bfg(q)}{dq}\quad+\bfLmd\bfg(q)\bigg)^T\mathbb f(q)dq\nonumber\\
&=0.
\label{Eq_Lg1}
\end{align}
%Since \eqref{Eq_Lg1} has to hold for all $g$ smooth in $q$, a necessary condition is that the coefficients of $\partial g/\partial q$ vanish:

%\begin{lmm}
%If \eqref{Eq_Lg1} holds, then $(\phi(i,0)-r(\phi,i,0))\sfz_i=0$ for all $i$.
%\label{Lmm_Fp}
%\end{lmm}
%\begin{proof}
%%We need to show that $(\phi(i,0)-r(\phi,i,0))\sfz_i=0$ for all $i$.
%Assume by contradiction that there exists $j\in\I$ such that $(\phi(i,0)-r(\phi,i,0))\sfz_j>0$ (note that $\phi(i,0)\ge r(\phi,i,0)$ for any $i$).
%Then, one can show that, if \eqref{Eq_Lg1} holds for both $g_1({i},q)=q$ and $g_2$ defined as
%\begin{align*}
%g_2({i},q)=\left\{\begin{array}{ll}
%2q, & {i}=j,\\
%q, & o.w.,
%\end{array}
%\right.
%\end{align*}
%then we can deduce from \eqref{Eq_Lg1} that
%\begin{align*}
%(\phi(j,0)-r(\phi,j,0))\sfz_j+\int_{q=0}^\infty (\phi(j,q)-r(\phi,j,q))\sff_j(q)dq=0,
%\end{align*}
%which cannot be true, since the first term is (by assumption) positive and the second term is non-negative.
%\end{proof}

Without computation, we can deduce that $(\phi(i,0)-r(\phi,i,0))\sfz_i=0$ for all $i$. The reason is as follows.
Let $\I_1=\{{i}\in\I:u^i>\phi(i,0)\}$ and $\I_2=\{{i}\in\I:u^i< \phi(i,0)\}$; $\I_1$ is the set of modes where the queue decreases, while $\I_2$ is the set of modes where the queue grows. 
%We can conclude from Lmm.~\ref{Lmm_Fp} that $\sfz_i=0$ if ${i}\in\I_2$. 
It is intuitive that there must be a growing queue when $f>u^i$. Therefore, $\sfz_i=0$ for all $i\in\I_2$.
If $\I=\I_1$, the solution will be trivial: $\sfz_i=\sfp_{i}$ and $\sff_{i}=0$ for all ${i}\in\I$.
Further characterization of $p_{\phi}$ in the general case is still an open question. However, we are able to analytically derive $p_{\phi}$ for BPDQs.

\begin{proof}[Proof of Prop. \ref{Prp_Inv}]
Since $u^2<f<u^1$, the previous argument in this section implies that $\sfz_1>0$ and $\sfz_2=0$. To compute $\sfz_1$, let $S_1(t)=\{\tau\in[0,t)|q(t)=0\}$, $\widetilde S_1(t)=\{\tau\in[0,t)|{i}(t)=1,q(t)>0\}$, and $\widetilde S_2(t)=\{\tau\in[0,t)|{i}(t)=2\}$. Without loss of generality, assume $q(0)=0$. Note that mass conservation gives
\begin{align*}
ft=S_1(t)f+\widetilde S_1(t)u^1+\widetilde S_2(t)u^2+q(t).
\end{align*}
By definitions of $\sfz_1$ and $\sfp_2$, and noting that $\sfz_2=0$ and that $q(t)$ is finite WP1 when $f<\ubar$, we have
\begin{align}
f&=\lim_{t\to\infty}\lb\frac{S_1(t)}tf+\frac{\widetilde S_1(t)}tu^1+\frac{\widetilde S_2(t)}tu^2+\frac{q(t)}t\rb\nonumber\\
&=\sfz_1f+\tilde\sfz_1u^1+\sfp_2u^2,\quad WP1,
\label{Eq_flim}
\end{align}
where $\tilde\sfz_1$ is the fraction of time when ${i}(t)=0$ and $q(t)>0$. By \eqref{Eq_p1p2}, we have
\begin{align}
\sfz_1+\tilde\sfz_1=\sfp_1=\frac{\mu}{\lambda+\mu},\quad
\sfp_2=\frac{\lambda}{\lambda+\mu}.
\label{Eq_p0}
\end{align}
Solving \eqref{Eq_flim}--\eqref{Eq_p0} for $\sfz_1$, we have
\begin{align*}
\sfz_1=\frac{1}{\lambda+\mu}\left(\mu-\lambda\frac{f-u^2}{u^1-f}\right).
\end{align*}

We now construct $\sff_1$ and $\sff_2$ taking the form $\sff_1=a_1e^{-sq}$ and $\sff_2=a_2e^{-sq}$, respectively, such that \eqref{Eq_sumLg} holds. Plugging the constructed $\sff_1$ and $\sff_2$ into \eqref{Eq_Lg1} and rearranging, we have
\begin{align}
&\sum_{{i}\in\I}\int_{dq\in\Q}\Ell g({i},q)p_f({i},dq)
=\lambda\Big(g(2,0)-g(1,0)\Big) \sfz_1\nonumber\\
&\;+\int_{q=0}^\infty\bigg((f-u^1)g'(1,q)+\lambda\Big(g(2,q)-g(1,q)\Big)\bigg)a_1e^{-sq}dq\nonumber\\
&\;+\int_{q=0}^\infty\bigg((f-u^2)g'(2,q)+\mu\Big(g(1,q)-g(2,q)\Big)\bigg)a_2e^{-sq}dq\nonumber\\
&=\Big(-\lambda \sfz_1-(f-u^1)a_2\Big)g(1,0)\nonumber\\
&\quad+\Big(\lambda \sfz_1-(f-u^2)a_2\Big)g(2,0)\nonumber\\
&\quad+\Big((f-u^1)a_1s+a_2\mu-a_1\lambda\Big)G(1,s)\nonumber\\
&\quad+\Big((f-u^2)a_2s+a_1\lambda-a_2\mu\Big)G(2,s),
\label{Eq_Ag2}
\end{align}
where $G(1,s)$ and $G(2,s)$ are Laplace transforms of $g(1,q)$ and $g(2,q)$. One can verify that $a_1$, $a_2$, and $s=1/\rho$ given by \eqref{Eq_a0}--\eqref{Eq_theta} vanish the coefficients of $g(1,0)$, $g(2,0)$, $G(1,s)$ and $G(2,s)$ in \eqref{Eq_Ag2}, and thus vanish \eqref{Eq_Ag2} for any $g$.%\footnote{For benchmarking of our derivation, we refer the readers to \cite{benaim14} for the analysis of a similar type of PDMPs .}
\end{proof}

\begin{proof}[Proof of Prop.~\ref{Prp_Inv_Bimodal}]
The proof follows from the proofs of Props.~\ref{Prp_Convergence2} and \ref{Prp_Inv} and Corr.~\ref{Cor_Queue} by replacing $f-u^1$ and $f-u^2$ with $\mathscr F_\min$ and $\mathscr F_\max$, respectively.
\end{proof}

\end{appendices}

\section*{Acknowledgment}
This work was supported by NSF CNS-1239054 CPS Frontiers: \underline{F}oundations \underline{O}f \underline{R}esilient \underline{C}yb\underline{E}r-Physical \underline{S}ystems (FORCES), NSF CAREER Award CNS-1453126, AFRL Lablet-Secure and Resilient Cyber-Physical Systems, and MIT CEE scholarship. We also appreciate valuable inputs from Prof. D. Teneketzis.

\bibliographystyle{ieeetr}
\bibliography{Bibliography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Jin.jpg}}]{Li Jin}
is a Ph.D. candidate in transportation at the Massachusetts Institute of Technology (MIT).  He received the B.Eng. degree from Shanghai Jiao Tong University (SJTU), China, in 2011, and the M.S. degree from Purdue University, West Lafayette, IN, in 2012, both in mechanical engineering.
His research area is resilient operations of transportation systems under unreliable capacities. He is interested in assessing negative impacts due to random failures in transportation networks and designing resilient control policies, using ideas from stochastic processes, dynamic control, and optimization.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Amin.png}}]{Saurabh Amin}
is Robert N. Noyce Career Development Assistant Professor in the Department of Civil and Environmental Engineering, Massachusetts Institute of Technology (MIT). His research focuses on the design and implementation of high confidence network control algorithms for infrastructure systems. He works on robust diagnostics and control problems that involve using networked systems to facilitate the monitoring and control of large-scale critical infrastructures, including transportation, water, and energy distribution systems. He also studies the effect of security attacks and random faults on the survivability of networked systems, and designs incentive-compatible control mechanisms to reduce network risks. Dr. Amin received his Ph.D. in Systems Engineering from the University of California, Berkeley in 2011. He is a recipient of NSF CAREER award, and Google Faculty Research award. 
\end{IEEEbiography}
